On the Lexical Distinguishability of Source Code

Natural language is robust against noise. The meaning of many sentences survives the loss of words, sometimes many of them. Some words in a sentence, however, cannot be lost without changing the meaning of the sentence. We call these words "wheat" and the rest "chaff". The word "not" in the sentence "I do not like rain" is wheat and "do" is chaff. For human understanding of the purpose and behavior of source code, we hypothesize that the same holds. To quantify the extent to which we can separate code into "wheat" and "chaff", we study a large (100M LOC), diverse corpus of real-world projects in Java. Since methods represent natural, likely distinct units of code, we use the ~9M Java methods in the corpus to approximate a universe of "sentences." We extract their wheat by computing the function's minimal distinguishing subset (Minset). Our results confirm that functions contain work offers the first quantitative evidence for recent promising work on keyword-based programming and insight into how to develop a powerful, alternative programming model.

==> lake/Rakefile <==
require 'fileutils'
require 'rake/clean'
require 'rake'
require 'set'

__DIR__ = File.expand_path( File.dirname( __FILE__) )

require File.join(__DIR__, 'util')
require File.join(__DIR__, 'latex_errors')

# Ruby 1.9.x is sensitive to file encodings and errors when reading latex source
# files, usually bibtex files, that contain non-ASCII characters.
Encoding.default_external = "UTF-8" if RUBY_VERSION =~ /1\.9\./

$MD5SUM = `which md5sum`.chomp
$MD5SUM = `which md5`.chomp if `uname` =~ /Darwin/

verbose(false) # Quiet the chatty shell commands.

if ENV['TEXINPUTS'].nil? or  ENV['TEXINPUTS'].empty?
	ENV['TEXINPUTS'] = "#{__DIR__}/packages/todos/::"
else
	ENV['TEXINPUTS'] = "#{__DIR__}/packages/todos/:" + ENV['TEXINPUTS']
end

TEX_FILES = FileList['*.tex']
MASTER_TEX_FILE_ROOTS = TEX_FILES.map do |f|
	f.chomp('.tex') unless `grep '^[[:space:]]*\\\\begin{document}' #{f}`.empty?
end.compact
error '
	No master (la)tex documents found:  no tex file contains \begin{document}.
'.strip.gsub(/^\t/,"") if MASTER_TEX_FILE_ROOTS.empty?

FIG_FILES = FileList['**/*.fig']
DIA_FILES = FileList['**/*.dia']

PDFTEX_FILES = FIG_FILES.map{|f| f.ext '.tex'}
DOT_FILES = FileList['**/*.dot']
NEATO_FILES = FileList['**/*.neato']
SECONDARY_PDF_FILES =
	DOT_FILES.map{|f| f.ext 'pdf'} \
	+ NEATO_FILES.map{|f| f.ext 'pdf'} \
	+ DIA_FILES.map{|f| f.ext 'pdf'}

GNUPLOT_DATA_FILES = FileList['**/*.gdata']
GNUPLOT_FILES = FileList['**/*.gplot'].map{|f| dot(f).ext 'gnuplot-output'}

# Local rakefiles must define R_CREATE_GRAPHS, the path to a script that
# generates pdfs from rdata files, in order for the rdata rules to take effect.
R_CREATE_GRAPHS = nil unless self.class.const_defined? :R_CREATE_GRAPHS
R_DATA_FILES = FileList['**/*.rdata']
R_FILES = R_DATA_FILES.map{|f| dot(f).ext 'r-output'}

# Ignore figures in excluded directories.
EXCLUDED_FIGURES = nil unless self.class.const_defined? :EXCLUDED_FIGURES

FIGURES = (PDFTEX_FILES + SECONDARY_PDF_FILES + GNUPLOT_FILES + R_FILES).
	reject { |f| f =~ EXCLUDED_FIGURES }

# Don't trash figures that are checked in directly (i.e. that we don't have the
# source for)
CLOBBER_EXTS = %w(pdf eps ps png Rout RData)
PREGENERATED_RESOURCES = FileList[
	`git ls-files`.split("\n").select do |f| 
		CLOBBER_EXTS.include? f[/\.(.*?)$/, 1]
	end
]

CLEAN.include(glob(%w(
	*.4ct *.4tc *.dvi *.idv *.lg *.lop *.lol *.toc *.out *.lof *.lot *.blg *.bbl
	*.lop *.loa *.tmp *.xref *.log *.aux *.vrb *.snm *.nav *.fls
)))
# Don't confuse .RData with the *.rdata files.  The former is detritus produced
# by the R binary.  
CLOBBER.include(
	glob(
		CLOBBER_EXTS.map{|ext| "**/*.#{ext}"}
	).reject{|f| f =~ EXCLUDED_FIGURES} - 
		glob('lake/**/*') +
		FIGURES - 
		PREGENERATED_RESOURCES
)
# Prevent latex from diverging while resolving references.
MAX_REFERENCE_RESOLUTIONS = 10


task :default => :view


def create_master_task(master)

	# Always refresh the fls and aux files so that get_deps_bibs_cites does not
	# return stale data, as when a dependency has been deleted; for this run, we
	# ignore errors.  This code accomplishes what -interaction nonstopmode
	# advertises, but fails to do.
	command = "pdflatex -draftmode -recorder -file-line-error '#{master}'"
	IO.popen( command, "w+" ) do |pipe|
		while line = pipe.gets
			# This regex may not capture all error prompts.
			pipe.puts "" if line =~ /^Enter|^\?/i
		end
	end

	# The deps variable includes figures, sty, cls, and package files: anything
	# latex reads when building the pdf.
	deps, bibs, cites = get_deps_bibs_cites master.ext("tex")

	# We delete the master.pdf task, which we are in, because we are going to
	# recreate it right here using the dependencies we just collected.  Then
	# we'll see if the redefined version needs to run.
	Rake.application.instance_variable_get('@tasks').delete(master.ext("pdf"))

	file master.ext('pdf') => deps + bibs + FIGURES + PREGENERATED_RESOURCES do

		# Run bibtex, if a bib file OR the set of cites has changed.
		if run_bibtex?( bibs, cites, master )
			# -min-crossrefs=100 essentially turns off cross referencing.
			# Not sure why one wouldn't just take the default of 2.
			sh "bibtex -terse -min-crossrefs=100 '#{master}'" 
		end

		options = [
			# be quiet and avoid interaction mode on error
			"-interaction batchmode",  
			# record files read and written during a build
			"-recorder",		  
			# output both file and line number on error
			"-file-line-error"	  
		]

		# At least one of the dependencies is newer, so run latex.
		puts "Running pdflatex..."
		system "pdflatex #{options.join( " " )} '#{master}' > /dev/null"
		if not $?.success?
			puts parse_log( File.read( master.ext( "log" ))).join( "\n\n" ) 
			exit 1
		end

		# Resolve references.
		i = 1
		prev_hash = `#{$MD5SUM} '#{master}.log'`
		cross_ref_regex = "(Rerun to get (citations|cross-references)"
		cross_ref_regex += "|Citation.*undefined)"
		while not `egrep -s '#{cross_ref_regex}' '#{master.ext("log")}'`.empty?

			puts "Re-running latex to resolve references."
			sh "pdflatex -interaction batchmode  '#{master}' > /dev/null"

			# Break if the log file has not changed or we exceed our 
			# resolution bound.
			hash = `#{$MD5SUM} '#{master}.log'`
			i += 1
			break if i > MAX_REFERENCE_RESOLUTIONS or prev_hash == hash

			prev_hash = hash

		end
		
		# Report citation keys that bibtex cannot find in the
		# imported bibliographic data (*.bib files).
		missing_cites = cites - get_bbl_keys([master.ext("bbl")])
		unless missing_cites.empty?
			msg = "The following bibtex key" \
				+ (missing_cites.size > 1 ? "s" : "")
			msg += " --- " + missing_cites.join(", ") 
			msg += " --- " + (missing_cites.size > 1 ? "were" : "was")
			msg += " not found in the imported file" \
				+ (bibs.size > 1 ? "s" : "")
			msg += ", " + bibs.join(", ") + ".\n"
			raise msg
		end
	end

	Rake::Task[master.ext("pdf")]
end

########################################################################
# Tasks to build the paper in various formats

desc "
	Builds the pdf output.  If the pdf is manually removed (i.e. not through the
	clean task), it may be necessary to call clobber before running this task.
".compact!
task :pdf  => MASTER_TEX_FILE_ROOTS.map{|master| master + '.pdf'}

# Rake does not currently support filering the dependency list of a rule to a
# subset of the files that share an extension.  Not all tex files are created
# equal; some tex files are "master" tex files that contain \begin{document} and
# input other tex files.  Here, we create a meta-task that creates (task, file)
# pairs for each master tex file in the project.
MASTER_TEX_FILE_ROOTS.each do |master|
	task master => master + '.pdf' # Don't make me type '.pdf'.

	# This meta-task creates tasks for each master, so that master task 
	# creation does not run every time this Rakefile is loaded, as when
	# one merely wishes to execute clean.
	task master.ext(".pdf") do
		master_task = create_master_task( master )
		master_task.invoke if master_task.needed? 
	end
end


desc <<-EOS
	Builds all of the figures
EOS
task :figures => FIGURES


rule '.tex' => ['.fig'] do |t|
	pdf_name = t.name.gsub /\.\w*$/, '.pdf'
	sh "fig2dev -Lpdftex -p0 #{t.source} > #{pdf_name} 2> /dev/null"
	sh "fig2dev -Lpdftex_t -p#{pdf_name} #{t.source} > #{t.name} 2> /dev/null"
end

rule '.pdf' => ['.eps'] do |t|
	sh "epstopdf #{t.source}"
end

rule '.eps' => ['.neato'] do |t|
	sh "neato -Gepsilon=.000000001 #{t.source} -Tps > #{t.name}"
end

rule '.eps' => ['.dot'] do |t|
	sh "dot #{t.source} -Tps > #{t.name}"
end

rule '.eps' => ['.dia'] do |t|
	sh "dia -t eps #{t.source}"
end

# Figures/.foo.gnuplot-output => Figures/foo.gplot
rule '.gnuplot-output' => proc{ |f|
	[undot(f).ext('gplot')] + GNUPLOT_DATA_FILES
} do |t|
	extension = gnuplot_target_extension(t.source)
	real_target_file = undot(t.name).ext extension
	sh "gnuplot < #{t.source} > #{real_target_file}"
	FileUtils.touch t.name
end

rule '.r-output' => proc{|f|
	[ undot(f).ext('rdata'), R_CREATE_GRAPHS].compact
} do |t|
	dir = File.dirname(t.name)
	repo_root = File.expand_path( File.join( __DIR__, '..'))
	sh "cd #{dir}; #{repo_root}/#{R_CREATE_GRAPHS} #{repo_root}/#{t.source}"
	FileUtils.touch t.name
end


########################################################################
# Task to view the paper
task :view => :pdf do
	viewer MASTER_TEX_FILE_ROOTS.first.ext("pdf")
end


==> lake/docs/bib_process <==

First latex run generates the \citation and \bibdata in the aux files.
These each occur only in the aux file of the corresponding .tex

First bibtex run reads aux files and created .bbl file containing the
\bibitem's for each citation.

First latex run after bibtex reads .bbl file and writes \bibcite commands
to aux file that contains \bibdata.  And puts the bibliography into pdf.

Second latex run after bibtex uses \bibcite commands to resolve citation numbers
in the pdf.



==> lake/macros/crossref.tex <==
%really these should be configurable on a per document basis, perhaps via 
%globals or should this be a template?  Anyway, the idea is to make it easy
% to shift back and forth between Figure and Fig. as required by the
% publisher's style.

%% cross references %%
\newcommand{\reffig}[1]{{Figure~\ref{#1}}}
\newcommand{\refthm}[1]{{Theorem~\ref{#1}}}
\newcommand{\refeq}[1]{{(\ref{#1})}}
\newcommand{\refalg}[1]{{Algorithm~\ref{#1}}}
\newcommand{\refex}[1]{{Example~\ref{#1}}}
\newcommand{\refsec}[1]{{Section~\ref{#1}}}


==> lake/macros/ps.tex <==
% Problem set macros. etb

\newboolean{@solutionset}

\newcommand{\answer}[1]{\ifthenelse{\boolean{@solutionset}}{{\sl #1}} {} }
\newcommand{\vanswer}[2]{\ifthenelse{\boolean{@solutionset}}{{\sl #1}}{\vspace*{#2mm}}}
\newcommand{\hanswer}[2]{\ifthenelse{\boolean{@solutionset}}{{\sl #1}}{\hspace*{#2mm}}}
\newcommand{\tanswer}[2]{\ifthenelse{\boolean{@solutionset}}{{\sl #1}} {#2} }
\newcommand{\zanswer}[1]{\ifthenelse{\boolean{@solutionset}}{{\sl #1}} {} }
\newcommand{\ifsol}[1]{ \ifthenelse{\boolean{@solutionset}} {#1} {} }
\newcommand{\ifthenelsesol}[2]{ \ifthenelse{\boolean{@solutionset}} {#1} {#2} }



==> lake/macros/symbols.tex <==
%% some symbols I use %%
\newcommand{\closeex}{\hfill$\triangle$}
\newcommand{\fallfact}[2]{{#1}^{\downarrow{#2}}}
\newcommand{\equal}[1]{{\:\stackrel{{\scriptscriptstyle\hspace{0.0em}(\sf{#1})}}{=}\:}}
\newcommand{\defeq}{{\:\stackrel{{\scriptscriptstyle\hspace{0.0em}\sf{def}}}{=}\:}}
\newcommand{\getsr}{{\:\stackrel{{\scriptscriptstyle\hspace{0.2em}\$}}{\leftarrow}\:}}
\newcommand{\andthen}{{\::\;\;}}    % \, \: \; for thinspace, medspace, thickspace
\newcommand{\Rand}[1]{{\sf{Rand}(\mbox{${#1}$})}}       % A command with one argument
\newcommand{\Perm}[1]{{\sf{Perm}(\mbox{${#1}$})}}
\newcommand{\Randd}[2]{{\mathrm{Rand}[{#1},{#2}]}} % and with two arguments
\newcommand{\given}{\mid}
\newcommand{\etwo}{{E^{(2)}}}


==> lake/packages/IEEETex/README <==

January 11, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

V1.7 is a significant update with many important changes. For a full list,
please read the file changelog.txt. The most notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> lake/packages/algorithm2e/algorithm2e_ex01.tex <==
\SetVline
\eIf{cond1}{
  a line\;
  a line\;
}{
  another line\;
  another line\;
}


==> lake/packages/algorithm2e/algorithm2e_ex02.tex <==
\SetNoline
\If{cond2}{
  second if\;
  second if\;
}


==> lake/packages/algorithm2e/algorithm2e_ex03.tex <==
\lIf{cond3}{ another example}
\Else{
  a block\;
  a block\;
}


==> lake/packages/algorithm2e/algorithm2e_ex04.tex <==
\lIf{cond4}{ok} \lElse{wrong}\;

==> lake/packages/algorithm2e/algorithm2e_ex05.tex <==
\SetVline
\lIf{cond5}{cond5 true}\;
\uElseIf{cond51}{
  cond 5 false\;
  but cond51 true\;
}
\ElseIf{}{
  all is wrong\;
  \Return result52\;
}


==> lake/packages/algorithm2e/algorithm2e_ex06.tex <==
\SetLine
\uIf{cond6}{
  cond6 is ok\;
  always ok\;
}
\uElseIf{cond62}{
  choose result62\;
  \Return result62\;
}
\Else{
  all is wrong\;
  do something else\;
}


==> lake/packages/algorithm2e/algorithm2e_ex07.tex <==
Let's have a look at what we can do
with if-then-else and side comments\;
\eIf{if-then-else test}{
  no comment here\;
  neither in then\;
}{
  nor in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  then with a comment\;
}(\tcc*[f]{comment in else})
{
  here we are in else\;
}
\eIf(\tcc*[f]{then comment}){test}{
  again a comment in then\;
}{
  but not in else\;
}
\eIf{if-then-else test}{
  this time, no comment in then\;
}(\tcc*[f]{else comment})
{
  but one comment in else\;
}
Let's try with other if possibilities\;
\lIf(\tcc*[h]{lif comment}){test}{text}
\uIf(\tcc*[f]{uif comment}){test}{
  then text\;
}
\uElseIf(\tcc*[f]{comment}){test}{
  elseif text\;
}
\lElseIf(\tcc*[h]{comment}){test}{text}
\lElse(\tcc*[f]{comment}){text}


==> lake/packages/algorithm2e/algorithm2e_exfor.tex <==
\SetLine
\ForAll{elements of $S_1$}{
  remove an element e from $S_1$\;
  put e in the set $S_2$\;
  }
\lFor{i=1 \emph{\KwTo}max}{mark i}\;
\ForEach{$e$ in the set}{
  put $e$ in ${\cal E}$\;
  mark $e$\;
}


==> lake/packages/algorithm2e/algorithm2e_exrepeat.tex <==
\Repeat{this stop condition}{
  the text of the loop\;
  another line\;
  always in the loop\;
  }
\lRepeat{stop}{a one line loop}


==> lake/packages/algorithm2e/algorithm2e_exswitch.tex <==
\Switch{the value of T}{
  \uCase{a value}{
    do this\;
    do that\;
  }
  \lCase{another value}{one line}\;
  \Case{last value}{
    do this\;
    break\;
  }
  \Other{
    for the other values\;
    do that\;
  }
}


==> lake/packages/ledmac/README <==
    The ledmac package is for typesetting critical editions. It is a
LaTeX port, and extension, of the plain TeX EDMAC, TABMAC and EDSTANZA
macros. The ledpar package is an extension of ledmac enabling parallel
typesetting in columns or on facing pages. The ledarab package is
an extension enabling the use of arabic script, as implemented by ArabTeX, 
in critical editions (temporarily afoot.sty is provided to support regular 
footnotes in ArabTeX).

    Bug reports and suggestions may be welcome.

Changes in ledpar.sty v0.3b (2005/04/08)
o Improved page balancing for parallel pages

Changes in ledpar.sty v0.3a (2005/03/30)
o Small fix for line number margins

Changes in ledarab.sty v0.1 (2005/03/24)
o First public release

Changes in ledpar version 0.3 (2005/03/24)
o Fixed some spacing problems
o Reorganized to simplify the ledarab package

Changes in ledpatch.sty v0.3 (2005/03/24)
o All patches incorporated into ledmac v0.7

Changes in ledmac version 0.7 (2005/03/24)
o Reorganized to simplify the ledpar and ledarab packages

Changes in ledpar version 0.2 (2005/01/01)
o Fixed problems with babel

Changes in ledpatch.sty v0.2 (2005/01/11)
o Fixed some spacing problems

Changes in ledpar version 0.1 (2004/12/10)
o First public release

Changes in ledmac version 0.6 (2004/12/10)
o Fixed infinite loop problems when processing complex paragraphs
o Prepared for the ledpar package

Changes in version 0.51 (2004/04/10)
o Resurrected line numbers in right hand margin
o Added a third kind of sidenote

Changes in version 0.5 (2004/04/04)
o Added sidenotes (as a replacement for \marginpar in numbered text)
o All footnotes can be used in numbered text, not just critical ones
o If used with the memoir class, multiple regular and critical indexes

Changes in version 0.4 (2004/02/29)
o Added draft/final options
o All footnotes can be used in minipages
o New minipage-like environments that can include page breaks and put 
  footnotes at their end, even if this is in the middle of the page
o Revised "ledeasy" example

Changes in version 0.3 (2004/02/14)
o Added edstanza macros for verse
o Line numbering can use roman, etc., numbers as well as arabic
o Additional example

Changes in version 0.22 (2003/11/09)
o More control over paragraphed footnotes
o More control over page and line number printing in footnotes
o Additional example
o Eliminated clash with the amsfonts package

Changes in version 0.21 (2003/09/13)
o Minor bug fixes
o Compatible with the memoir class (mempatch v1.8)

Changes in version 0.2 (2003/08/16)
o Added indexing by page and line number
o Added simple tabular- and array-style environments

Changes in version 0.1 (2003/03/25)
o First public experimental release.

-------------------------------------------------------------------- 
  Author: Peter Wilson (Herries Press) herries dot press at earthlink dot net
  Copyright 2003 --- 2005 Peter R. Wilson
 
  This work may be distributed and/or modified under the
  conditions of the LaTeX Project Public License, either
  version 1.3 of this license or (at your option) any 
  later version.
  The latest version of the license is in
     http://www.latex-project.org/lppl.txt
  and version 1.3 or later is part of all distributions of
  LaTeX version 2003/06/01 or later.
 
  This work has the LPPL maintenance status "author-maintained".
 
  This work consists of the files:
   README (this file), 
   ledmac.dtx, 
   ledmac.ins,
   ledmac.pdf   (200+ pages)
   ledeasy.eps, 
   ledfeat.eps, 
   ledioc.eps, 
   ledarden.eps, 
   ledmixed.eps,
   ledekker.eps, 
   ledbraonain.eps,
   ledpar.dtx,
   ledpar.ins,
   ledpar.pdf   (100+ pages)
   djd17novL.eps,
   djd17novR.eps,
   djdpoems1.eps,
   djdpoems2.eps,
   djdpoems3.eps,
   djdpoems4.eps,
   villon.eps,
   ledarab.dtx,
   ledarab.ins,
   ledarab.pdf (20- pages)
   egarab.eps
   egarabpar.eps
   ledpatch.sty
   ledparpatch.sty
   ledarabpatch.sty
and the derived files 
   ledmac.sty, 
   ledeasy.tex, 
   ledfeat.tex, 
   ledioc.tex, 
   ledarden.tex,
   ledmixed.tex,
   ledekker.tex, 
   ledbraonain.tex,
   ledpar.sty,
   djd17nov.tex,
   djdpoems.tex, 
   villon.tex,
   ledarab.sty
   egarab.tex
   egarabpar.tex
   afoot.sty

-------------------------------------------------------------------- 

    The distribution consists of the following files:
README (this file)
ledmac.dtx
ledmac.ins
ledmac.pdf
ledeasy.eps
ledfeat.eps
ledioc.eps
ledarden.eps
ledmixed.eps
ledekker.eps
ledbraonain.eps
ledpar.dtx
ledpar.ins
ledpar.pdf
djd17novL.eps
djd17novR.eps
djdpoems1.eps
djdpoems2.eps
djdpoems3.eps
djdpoems4.eps
villon.eps
ledarab.dtx
ledarab.ins
ledarab.pdf
egarab.eps
egarabpar.eps
(possibly ledpatch.sty)
(possibly ledparpatch.sty)
(possibly ledarabpatch.sty)


    To install the ledmac package:
o run: latex ledmac.ins (which will generate ledmac.sty)
o Move ledmac.sty (and ledpatch.sty if it exists) to a location where 
  LaTeX will find it (for more information on this see the FAQ).

    To generate a second copy of the manual (which is already supplied as a PDF file):
o run: latex ledmac.dtx
o (for an index run: makeindex -s gind.ist ledmac)
o run: latex ledmac.dtx
o Print ledmac.dvi for a hardcopy of the package manual 

    The *.eps files are example pages processed with the ledmac package.
They are included as figures in ledmac.dtx, which also contains the
source code for them.

    Installation of the other packages (via ledpar.ins and ledarab.ins)
is similar.
 
2005/04/08
Peter Wilson
herries dot press at earthlink dot net




==> lake/packages/oz/objectz/readme <==
This is a revision of Paul King's oz.sty macros for typesetting Object Z,
updated for LaTeX2e. Users should run ozguide.tex through \LaTeX\ (after
installation!) for details of usage.

Install by running \TeX\ on oz.ins and install oz.sty where \LaTeX\
can find it.

UPDATE NOVEMBER 1996
********************

The Formal Methods Group in the Computer Science Department at the
University of Queensland recently released 'wizard', a type checker
for Object-Z specifications.  Included in the wizard release was an
updated version of the oz.sty file for LaTeX 2.09.

I have implemented all changes made in the oz.sty for LaTeX 2.09,
since it's last official release in late 1990, into the oz.dtx file
which you maintain for LaTeX 2e.  I have attached my updated version
of oz.dtx to this message so that you may check these modifications
and officially release the updated version.

The changes were made to the oz.dtx file with last changes logged
on 22 Feb 95 (this is the version currently available from CTAN).
All modifications and additions I have made are clearly indicated in
the updated file for your convenience.

Should you need to compare my changes with the updated oz.sty file for
LaTeX 2.09, you can download the wizard archive from the following url:

	ftp://ftp.cs.uq.edu.au/pub/SVRC/software/wizard.tar.gz

The new oz.sty file and oz.tex file are located in the wizard/tex
subdirectory when the archive is extracted.

Please contact me if you need to.

Thanks.

Dave.
--
David Leadbetter                                    Email: davidl@cs.uq.edu.au
PhD Student                                         Phone: + 61 7 3365 1204
Department of Computer Science                      FAX:   + 61 7 3365 1999
The University Of Queensland 4072 AUSTRALIA



==> lake/packages/oz/readme <==
This is a revision of Paul King's oz.sty macros for typesetting Object Z,
updated for LaTeX2e. Users should run ozguide.tex through \LaTeX\ (after
installation!) for details of usage.

Install by running \TeX\ on oz.ins and install oz.sty where \LaTeX\
can find it.

UPDATE NOVEMBER 1996
********************

The Formal Methods Group in the Computer Science Department at the
University of Queensland recently released 'wizard', a type checker
for Object-Z specifications.  Included in the wizard release was an
updated version of the oz.sty file for LaTeX 2.09.

I have implemented all changes made in the oz.sty for LaTeX 2.09,
since it's last official release in late 1990, into the oz.dtx file
which you maintain for LaTeX 2e.  I have attached my updated version
of oz.dtx to this message so that you may check these modifications
and officially release the updated version.

The changes were made to the oz.dtx file with last changes logged
on 22 Feb 95 (this is the version currently available from CTAN).
All modifications and additions I have made are clearly indicated in
the updated file for your convenience.

Should you need to compare my changes with the updated oz.sty file for
LaTeX 2.09, you can download the wizard archive from the following url:

	ftp://ftp.cs.uq.edu.au/pub/SVRC/software/wizard.tar.gz

The new oz.sty file and oz.tex file are located in the wizard/tex
subdirectory when the archive is extracted.

Please contact me if you need to.

Thanks.

Dave.
--
David Leadbetter                                    Email: davidl@cs.uq.edu.au
PhD Student                                         Phone: + 61 7 3365 1204
Department of Computer Science                      FAX:   + 61 7 3365 1999
The University Of Queensland 4072 AUSTRALIA



==> lake/preamble-llncs.tex <==
\usepackage{graphicx,color}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm} %incompatible with sig-alternate
\usepackage{url} % do I need this with hyperref?
\usepackage{multicol}
\usepackage{multirow}
%\usepackage{setspace} % for double, 1.5, single spacing etc.
% setspace messes up the line numbering of algorithmic
\usepackage{xspace}
\usepackage{listings}
\usepackage{ifthen}
\usepackage{verbatim}
\usepackage{float} % defines newfloat used below
\usepackage{microtype}
\usepackage{fixltx2e} 

% These two let you use multibyte utf-8 characters, e.g. 03bb - λ 
\usepackage[mathletters]{ucs}
\usepackage[utf8x]{inputenc}

% hyperref redefines a number of macros, so it should be last.  Empirically,
% doing so eliminates compiler warnings.
\usepackage[%
	bookmarks, colorlinks, citecolor=green, urlcolor=blue,
	filecolor=blue, linkcolor=blue, pdfpagelabels=false%
]{hyperref}
\usepackage{algorithmic} % may not be installed
\usepackage{algorithm}

% required for combined latex/pdf xfig figures
\DeclareGraphicsRule{.pdftex}{pdf}{.pdftex}{} 


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Macros																{{{1

% English
\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\scil}{\hbox{\emph{sc.}}\xspace} %scilicet: it is permitted to know
\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace} %videlicet: it is permitted to see


\newfloat{Protocol}{thp}{lop}
\DeclareMathOperator{\cbar}{||} %denotes concurrency in protocol floats.
\newfloat{Program}{thp}{lop}
\newfloat{Procedure}{thp}{lop}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Theorems, etc.														{{{2
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\bigskip}

%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}

%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Aliases																{{{1
\newcommand{\infinity}{\infty}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~





% vim:foldmethod=marker


==> lake/preamble-sigalt.tex <==
\usepackage{graphicx,color}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{url} % do I need this with hyperref?
\usepackage{multicol}
\usepackage{multirow}
%\usepackage{setspace} % for double, 1.5, single spacing etc.
% setspace messes up the line numbering of algorithmic
\usepackage{xspace}
\usepackage{listings}
\usepackage{ifthen}
\usepackage{verbatim}
\usepackage{float} % defines newfloat used below
\usepackage{microtype}
\usepackage{mathptmx}
\usepackage{stmaryrd} %Additional math symbols.
\usepackage{textcomp}
\usepackage[sort&compress]{natbib}
\usepackage{todos} % Use \todoset{all=off} to turn off todos in a paper.
\usepackage{fixltx2e} 
\usepackage{booktabs}
\usepackage{fancyhdr}

% These two let you use multibyte utf-8 characters, e.g. 03bb - λ 
\usepackage[mathletters]{ucs}
\usepackage[utf8x]{inputenc}
\usepackage{wasysym}	% Defines \cent, \currency, \brokenvert

% hyperref redefines a number of macros, so it should be last.  Empirically,
% doing so eliminates compiler warnings.
\usepackage[%
	bookmarks, colorlinks, citecolor=green, urlcolor=blue,
	filecolor=blue, linkcolor=blue, pdfpagelabels=false%
]{hyperref}
\usepackage{algorithmic} % may not be installed
\usepackage{algorithm}

% required for combined latex/pdf xfig figures
\DeclareGraphicsRule{.pdftex}{pdf}{.pdftex}{} 


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Macros																{{{1

% English
\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\scil}{\hbox{\emph{sc.}}\xspace} %scilicet: it is permitted to know
\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace} %videlicet: it is permitted to see


\newfloat{Protocol}{thp}{lop}
\DeclareMathOperator{\cbar}{||} %denotes concurrency in protocol floats.
\newfloat{Program}{thp}{lop}
\newfloat{Procedure}{thp}{lop}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Theorems, etc.														{{{2
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\bigskip}

%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}

%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Aliases																{{{1
\newcommand{\infinity}{\infty}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~





% vim:foldmethod=marker


==> preamble-sigalt.tex <==
\usepackage{graphicx,color}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{amsthm}
\usepackage{url} % do I need this with hyperref?
\usepackage{multicol}
\usepackage{multirow}
%\usepackage{setspace} % for double, 1.5, single spacing etc.
% setspace messes up the line numbering of algorithmic
\usepackage{xspace}
\usepackage{listings}
\usepackage{ifthen}
\usepackage{verbatim}
\usepackage{float} % defines newfloat used below
\usepackage{microtype}
\usepackage{mathptmx}
\usepackage{stmaryrd} %Additional math symbols.
\usepackage{textcomp}
\usepackage[sort&compress]{natbib}
\usepackage{todos} % Use \todoset{all=off} to turn off todos in a paper.
\usepackage{fixltx2e} 
\usepackage{booktabs}
\usepackage{fancyhdr}

% These two let you use multibyte utf-8 characters, e.g. 03bb - λ 
\usepackage[mathletters]{ucs}
\usepackage[utf8x]{inputenc}
\usepackage{wasysym}	% Defines \cent, \currency, \brokenvert

% hyperref redefines a number of macros, so it should be last.  Empirically,
% doing so eliminates compiler warnings.
\usepackage[%
	bookmarks, colorlinks, citecolor=green, urlcolor=blue,
	filecolor=blue, linkcolor=blue, pdfpagelabels=false%
]{hyperref}
\usepackage{algorithmic} % may not be installed
\usepackage{algorithm}

% required for combined latex/pdf xfig figures
\DeclareGraphicsRule{.pdftex}{pdf}{.pdftex}{} 


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Macros																{{{1

% English
\newcommand{\cf}{\hbox{\emph{cf.}}\xspace}
\newcommand{\deletia}{\ldots [deletia] \ldots}
\newcommand{\etal}{\hbox{\emph{et al.}}\xspace}
\newcommand{\eg}{\hbox{\emph{e.g.}}\xspace}
\newcommand{\ie}{\hbox{\emph{i.e.}}\xspace}
\newcommand{\scil}{\hbox{\emph{sc.}}\xspace} %scilicet: it is permitted to know
\newcommand{\st}{\hbox{\emph{s.t.}}\xspace}
\newcommand{\wrt}{\hbox{\emph{w.r.t.}}\xspace}
\newcommand{\etc}{\hbox{\emph{etc.}}\xspace}
\newcommand{\viz}{\hbox{\emph{viz.}}\xspace} %videlicet: it is permitted to see


\newfloat{Protocol}{thp}{lop}
\DeclareMathOperator{\cbar}{||} %denotes concurrency in protocol floats.
\newfloat{Program}{thp}{lop}
\newfloat{Procedure}{thp}{lop}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Theorems, etc.														{{{2
\newenvironment{proof-idea}{\noindent{\bf Proof Idea}\hspace*{1em}}{\bigskip}

%\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}

%\theoremstyle{remark}
%\newtheorem*{rem}{Remark}

%\theoremstyle{definition}
\newtheorem{defn}{Definition}[section]
\newtheorem{conj}{Conjecture}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
% Aliases																{{{1
\newcommand{\infinity}{\infty}
%}}}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~





% vim:foldmethod=marker


==> todos.tex <==
%\section{Todos}
%\label{sec:todos}
%
%\begin{enumerate}[(1)]
%\item We can also do a small-scaled analysis on C (C++) to see whether the
%distribution of function size is similar with Java.
%
%\item Set up the framework of automatically and preciously extracting function
%and keywords from Java source code. (Currently I use \textit{Eclipse JDT API} to
%extract information from source code by static analysis)
%\item We may also need to set up the similar framework for C and C++. (Eclipse
%CDT API might be a candidate for extracting keyword-related information from C
%and C++ source code. Any other optional choice?)
%\item Implement the algorithm of keyword minimal set selection.
%\end{enumerate}
%

